Tackling Multipath and Biased Training Data for IMU-Assisted BLE Proximity Detection

Proximity detection is to determine whether an IoT receiver is within a certain distance from a signal transmitter. Due to its low cost and high popularity, Bluetooth low energy (BLE) has been used to detect proximity based on the received signal strength indicator (RSSI). To address the fact that RSSI can be markedly influenced by device carriage states, previous works have incorporated RSSI with inertial measurement unit (IMU) using deep learning. However, they have not sufficiently accounted for the impact of multipath. Furthermore, due to the special setup, the IMU data collected in the training process may be biased, which hampers the system's robustness and generalizability. This issue has not been studied before. We propose PRID, an IMU-assisted BLE proximity detection approach robust against RSSI fluctuation and IMU data bias. PRID histogramizes RSSI to extract multipath features and uses carriage state regularization to mitigate overfitting due to IMU data bias. We further propose PRID-lite based on a binarized neural network to substantially cut memory requirements for resource-constrained devices. We have conducted extensive experiments under different multipath environments, data bias levels, and a crowdsourced dataset. Our results show that PRID significantly reduces false detection cases compared with the existing arts (by over 50%). PRID-lite further reduces over 90% PRID model size and extends 60% battery life, with a minor compromise in accuracy (7%).

==> sections/discussion.tex <==
% Generalization ability depends on training data
% IMU cannot 100% reflects carriage state influences
% heterogeneity

% {\LARGE FOR A SINGLE SMALL SECTION LIKE THIS, YOU DO NOT NEED TO BIRD'S EYE REVIEW IT.
% This section discusses some further considerations on BLE proximity detection that need to be addressed in the future.}
Firstly, current BLE proximity detection leverages data-driven methods to acquire adaptation on diverse multipath environments.
Thus, {\LARGE ISN'T THIS CASE CONSIDERED AS BIASED TRAINING DATA? it assumes that training and test data (in terms of RSSI) should be drawn from the same distribution. }
However, it is possible that BLE proximity detection is conducted in a new {\LARGE IS THIS OOD?  HOW DOES OOD DIFFER FROM YOUR BIAS? YOU MAY WANT TO DISCUSS IT IN YOUR RELATED WORK SECTION AND ARGUE WHY THE WORK THERE IS NOT APPLICABLE HERE environment whose signal distribution is not covered in training data.}
So this out-of-distribution issue needs to be studied in the future.
Secondly, existing works on BLE proximity detection use IMU to reflect carriage state.
However, device pose only marginally reflects carriage state impact on BLE signals.
For example, RSSI could even be different with different clothing materials under the device pose of "in pocket."
Therefore, more sensors should be studied in the future.
Thirdly, we only consider the receiver's carriage state in this paper. 
For the transmitter, its carriage feature can be extracted similarly and conveyed via the BLE message in implementation.
{\LARGE THIS SECTION WAS NOT WRITTEN WELL OR CLEARLY.  SHOULD IT BE MOVED TO BE WITH CONCLUSION AS A LAST PARAGRAPH OF FUTURE WORKS?}

